Observations, Thermochemical Calculations, and Modeling of Exoplanetary Atmospheres

This dissertation as a whole aims to provide means to better understand hot-Jupiter planets through observing, performing thermochemical calculations, and modeling their atmospheres. We used Spitzer multi-wavelength secondary-eclipse observations and targets with high signal-to-noise ratios, as their deep eclipses allow us to detect signatures of spectral features and assess planetary atmospheric structure and composition with greater certainty. Chapter 1 gives a short introduction. Chapter 2 presents the Spitzer secondary-eclipse analysis and atmospheric characterization of WASP-14b. WASP-14b is a highly irradiated, transiting hot Jupiter. By applying a Bayesian approach in the atmospheric analysis, we found an absence of thermal inversion contrary to theoretical predictions. Chapter 3 describes the infrared observations of WASP-43b Spitzer secondary eclipses, data analysis, and atmospheric characterization. WASP-43b is one of the closest-orbiting hot Jupiters, orbiting one of the coolest stars with a hot Jupiter. The atmospheric analysis ruled out a strong thermal inversion in its dayside atmosphere. Chapter 4 presents an open-source Thermochemical Equilibrium Abundances (TEA) code and its application to several hot Jupiters. TEA calculates the abundances of gaseous species using the Gibbs free-energy minimization method within an iterative Lagrangian optimization scheme. The code is written in Python and available to the community via http://github.com/dzesmin/TEA. Chapter 5 presents my contributions to an open-source Bayesian Atmospheric Radiative Transfer (BART) code, and its application to WASP-43b. BART characterizes planetary atmospheres based on the observed spectroscopic information. It initializes a planetary atmospheric model, performs radiative-transfer calculations to produce models of planetary spectra, and using a statistical module compares models with observations.

==> latbibucf <==
#! /bin/bash

root=$1

if [ -d /usr/share/texmf-texlive ]; then
  tex_dir=/usr/share/texmf-texlive
else
  tex_dir=/usr/share/texmf-tetex
fi

export TEXFONTS=.:/home/jh/lib/texmf/fonts//:${tex_dir}/fonts//
export TEXINPUTS=.:/home/jh/lib/texmf/tex//:${tex_dir}/tex//
export BIBINPUTS=.:/home/jh/ast/papers/bib//:/home/jh/lib/texmf/bibtex/bib//:${tex_dir}/bibtex/bib//
export BSTINPUTS=.:/home/jh/lib/texmf/bibtex/bst//:${tex_dir}/bibtex/bst//
export DVIPSFONTS=${TEXFONTS}:/var/lib/texmf//

# latexcl
rm -f *.bbl \
      *.blg \
      *.dvi \
      *.log \
      *.aux \
      *.ps \
      *.out \
      *.toc \
      *.lot \
      *.lof

# lblll
latex ${root}
bibtex ${root}
for auxfile in chap*.aux
do
    bibtex `basename $auxfile .aux`
done
latex ${root}
latex ${root}
latex ${root}

dvipdfm ${root}
#pdflatex ${root}

#Manually rotate necessary pages with Applications -> Graphics -> PDF Editor

# latpdf
#dvips -P pdf -f ${root} | \
#  ps2pdf -dMaxSubsetPct=100 -dCompatibilityLevel=1.4 \
#         -dSubsetFonts=true -dEmbedAllFonts=true - - \
#> ${root}.pdf

